Patchy Forsterite Clouds in the Atmospheres of Two Highly Variable Exoplanet Analogs

We present an atmospheric retrieval analysis of a pair of highly variable, $\sim200~$Myr old, early-T type planetary-mass exoplanet analogs SIMP J01365662+0933473 and 2MASS J21392676+0220226 using the Brewster retrieval framework. Our analysis, which makes use of archival $1-15~\mu$m spectra, finds almost identical atmospheres for both objects. For both targets, we find that the data is best described by a patchy, high-altitude forsterite (Mg$_2$SiO$_4$) cloud above a deeper, optically thick iron (Fe) cloud. Our model constrains the cloud properties well, including the cloud locations and cloud particle sizes. We find that the patchy forsterite slab cloud inferred from our retrieval may be responsible for the spectral behavior of the observed variability. Our retrieved cloud structure is consistent with the atmospheric structure previously inferred from spectroscopic variability measurements, but clarifies this picture significantly. We find consistent C/O ratios for both objects which supports their formation within the same molecular cloud in the Carina-Near Moving Group. Finally, we note some differences in the constrained abundances of H$_2$O and CO which may be caused by data quality and/or astrophysical processes such as auroral activity and their differing rotation rates. The results presented in this work provide a promising preview of the detail with which we will characterize extrasolar atmospheres with JWST, which will yield higher quality spectra across a wider wavelength range.

==> 2M2139+SIMP0136 Retrieval/0136_2139_BICs.tex <==
\begin{table*}[tb]
\begin{tabular}{llll}
Model                  & $N$ Params           &\obj{s0136}   &  \obj{2m2139}\\     
                       &                      &$\Delta$~BIC  &$\Delta$~BIC\\ \hline    
Patchy Forsterite Slab \& Iron Deck & 32      & 0            & 0\\
Forsterite Slab \& Iron Deck  & 31            & 118          & 8\\
Enstatite Slab \& Iron Deck  & 31             & 119          &10\\
Patchy Enstatite Slab \& Iron Deck & 32       & 77           & 19\\
Forsterite Slab        & 27                   & 105          &20   \\
Iron Deck              & 26                   & 104          &38  \\
%SiO Slab              & 25                    & 39           & 47\\
Enstatite Slab         & 27                   & 140          & 52\\
Forsterite Deck        & 26                   & 123          &56\\
No clouds              & 22                   & 578          & 56 \\ 
Enstatite Deck         & 26                   & 131          & 59     \\
Iron Slab              & 26                   & 120          & 65\\ \hline  \hline  
\end{tabular}
\caption{List of models tested in this work for  \obj{s0136} and \obj{2m2139} along with $\Delta$BIC. Models are arranged in order of the most favored model to least favored model for \obj{2m2139}.}
\label{tab:0136_2139_BICS}
\end{table*}

==> 2M2139+SIMP0136 Retrieval/cloudparams.tex <==
\begin{deluxetable*}{lcccc}[tb]
\tabletypesize{\small}
\tablecolumns{10}
\tablewidth{0pt}
\setlength{\tabcolsep}{0.05in}
\tablecaption{Summary of retrieved cloud properties for the preferred models for \obj{s0136} and \obj{2m2139}.}
\label{tab:cloudprops}
\tablehead{  
\colhead{}&
\colhead{\obj{s0136}}&
\colhead{ }&
\colhead{\obj{2m2139}}&
\colhead{ }}
\startdata
Cloud No.                               & 1                          & 2                          &  1                        &  2 \\
Type                                    & Slab                       & Deck                       & Slab                      & Deck                  \\
Species                                 & Mg$_2$SiO$_4$                 & Fe                      & Mg$_2$SiO$_4$                 & Fe                    \\
Cloud Coverage                          & $0.70^{+0.03}_{-0.04}$     &n/a                         &$0.83_{-0.06}^{+0.06}$        &n/a                       \\
Max $\tau_{\mathrm{cloud}}$ at $1~\mu$m & $12.03^{+1.03}_{-0.85}$    &n/a                         & $8.17_{-1.38}^{+1.54}$     &n/a                    \\
Reference Pressure / log$P$ (bar) & $0.24^{+0.06}_{-0.05}$ (max $\tau$) & $0.90^{+0.04}_{-0.05}$ ($\tau=1$)  & $0.12_{-0.09}^{+0.08}$ (max $\tau$)& $0.86_{-0.07}^{+0.09}$ ($\tau=1$)    \\
Height / $d$log$P$(bar)                      & $0.50^{+0.09}_{-0.096}$    & $0.06^{+0.03}_{-0.02}$     & $0.32_{-0.15}^{+0.20}$     & $0.03_{-0.02}^{+0.03}$     \\
Log(effective particle radius $a$/$\mu$m)        & $-1.47^{+0.14}_{-0.14}$  & $-1.35^{+0.25}_{-0.31}$    & $-1.21_{-0.19}^{+0.18}$    & $-1.31_{-0.66}^{+0.45}$     \\
Particle radius spread (Hansen distribution $b$) & $0.36^{+0.33}_{-0.25}$     & $0.51^{+0.33}_{-0.33}$     & $0.42_{-0.29}^{+0.34}$     & $0.52_{-0.35}^{+0.34}
$    
\enddata
\end{deluxetable*}

==> 2M2139+SIMP0136 Retrieval/gasabundances.tex <==
\begin{deluxetable}{lrr}[tb]
\tabletypesize{\small}
\tablecolumns{10}
\tablewidth{0pt}
\setlength{\tabcolsep}{0.05in}
\tablecaption{Summary of retrieved gas abundances for the preferred models for \obj{s0136} and \obj{2m2139}.}
\label{tab:gases}
\tablehead{  
\colhead{}&
\colhead{\obj{s0136}}&
\colhead{\obj{2m2139}}}
\startdata
H$_2$O      & $-4.03^{+0.03}_{-0.03}$         & $-3.84^{+0.07}_{-0.06}$          \\
CO          & $-3.60^{+0.06}_{-0.06}$         & $-3.24^{+0.10}_{-0.09}$          \\
CO$_2$      & $-7.00^{+0.06}_{-0.07}$         & $-4.87^{+0.15}_{-0.74}$          \\
CH$_4$      & $-4.64^{+0.05}_{-0.04}$         & $-4.65^{+0.10}_{-0.09}$          \\
NH$_3$      & $-6.09^{+0.12}_{-0.13}$         & $-5.64^{+0.15}_{-0.17}$          \\
CrH         & $-9.75^{+0.12}_{-0.13}$         & $-9.47^{+0.16}_{-0.16}$          \\
FeH         & $-9.33^{+0.06}_{-0.06}$         & $-9.68^{+0.14}_{-0.18}$          \\
SiO         & $-9.09^{+1.95}_{-1.97}$         & $-9.55^{+2.02}_{-1.59}$          \\
Na+K        & $-6.39^{+0.08}_{-0.08}$         & $-6.51^{+0.15}_{-0.15}$          \\
log(g)      & $4.25^{+0.08}_{-0.08}$          & $4.27^{+0.16}_{-0.13}$        
\enddata
\end{deluxetable}

==> 2M2139+SIMP0136 Retrieval/objects.tex <==
% Awesome system for defining object shorthands. First:
%
% \DefineObj[short name]{nickname}{long name}
%
% Then
%
% \obj*{nickname} => long name
% \obj{nickname} => short name if defined, otherwise long name
%
% The nicknames can include numbers, which is nice because LaTeX command names
% can't!

\makeatletter
\newcommand\DefineObj[3][\@empty]{%
  \expandafter\newcommand\csname pkgwobj@l#2\endcsname{#3}%
  \ifx\@empty#1%
    \expandafter\newcommand\csname pkgwobj@s#2\endcsname{#3}%
  \else%
    \expandafter\newcommand\csname pkgwobj@s#2\endcsname{#1}%
  \fi}%
\newcommand{\pkgw@printobj@long}[1]{%
  \expandafter\ifx\csname pkgwobj@l#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@l#1\endcsname%
  \fi}%
\newcommand{\pkgw@printobj@short}[1]{%
  \expandafter\ifx\csname pkgwobj@l#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@s#1\endcsname%
  \fi}%
\newcommand{\obj}{\@ifstar{\pkgw@printobj@long}{\pkgw@printobj@short}}%
\makeatother
